ACE: Anti-Editing Concept Erasure in Text-to-Image Models

Recent advance in text-to-image diffusion models have significantly facilitated the generation of high-quality images, but also raising concerns about the illegal creation of harmful content, such as copyrighted images. Existing concept erasure methods achieve superior results in preventing the production of erased concept from prompts, but typically perform poorly in preventing undesired editing. To address this issue, we propose an Anti-Editing Concept Erasure (ACE) method, which not only erases the target concept during generation but also filters out it during editing. Specifically, we propose to inject the erasure guidance into both conditional and the unconditional noise prediction, enabling the model to effectively prevent the creation of erasure concepts during both editing and generation. Furthermore, a stochastic correction guidance is introduced during training to address the erosion of unrelated concepts. We conducted erasure editing experiments with representative editing methods (i.e., LEDITS++ and MasaCtrl) to erase IP characters, and the results indicate that our ACE effectively filters out target concepts in both types of edits. Additional experiments on erasing explicit concepts and artistic styles further demonstrate that our ACE performs favorably against state-of-the-art methods. Our code will be publicly available at https://github.com/120L020904/ACE.

==> table/edit_erasure_IP.tex <==
\begin{table*}[ht]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|cc|cc|cc|cc|cc|cc}
    \hline
        ~ & \multicolumn{6}{c|}{LEDITS++}  & \multicolumn{6}{c}{MasaCtrl} \\ \hline
        ~ & \multicolumn{2}{c|}{Erase Concept}  & \multicolumn{2}{c|}{Prior Concept} & \multicolumn{2}{c|}{Overall} & \multicolumn{2}{c|}{Erase Concept} & \multicolumn{2}{c|}{Prior Concept} & \multicolumn{2}{c}{Overall} \\
        ~ & $\text{CLIP}_e\downarrow$ & $\text{LPIPS}_e\uparrow$ & $\text{CLIP}_p\uparrow$ & $\text{LPIPS}_p\downarrow$ & $\text{CLIP}_d\uparrow$ & $\text{LPIPS}_d\uparrow$& $\text{CLIP}_e\downarrow$ & $\text{LPIPS}_e\uparrow$ & $\text{CLIP}_p\uparrow$ & $\text{LPIPS}_p\downarrow$ & $\text{CLIP}_d\uparrow$ & $\text{LPIPS}_d\uparrow$ \\ \hline 
        Original & 0.312 & 0.000 & 0.312 & 0.000 & 0.000 & 0.000 & 0.312 & 0.000 & 0.312 & 0.000 & 0.000 & 0.000 \\
        SD v1.4~\cite{rombach2022high} & 0.308 & 0.063 & 0.308 & 0.063 & 0.000 & 0.000 & 0.312 & 0.152 & 0.312 & 0.152 & 0.000 & 0.000 \\ \hline
        ESD~\cite{gandikota2023erasing} & 0.306 & 0.042 & 0.307 & 0.041 & 0.001 & 0.000 & 0.293 & 0.179 & 0.307 & 0.157 & 0.015 & 0.022 \\
        SPM~\cite{lyu2024one} & 0.302 & 0.061 & 0.303 & 0.056 & 0.001 & 0.005 & 0.293 & 0.192 & 0.311 & 0.154 & 0.018 & 0.038 \\
        AdvUnlearn~\cite{zhang2024defensive} & 0.310 & 0.011 & \textbf{0.311} & \textbf{0.010} & 0.001 & 0.001 & 0.245 & 0.246 & 0.303 & \textbf{0.148} & 0.058 & 0.099 \\
        MACE~\cite{lu2024mace} & 0.303 & 0.056 & 0.304 & 0.054 & 0.001 & 0.002 & 0.297 & 0.184 & \textbf{0.312} & 0.151 & 0.014 & 0.033 \\ 
        RECE~\cite{gong2024reliable} & 0.300 & 0.066 & 0.303 & 0.054 & \underline{0.003} & \underline{0.012} & 0.238 & 0.266 & 0.302 & 0.167 & \underline{0.065} & \underline{0.100} \\ 
        Ours & \textbf{0.274} & \textbf{0.168} & 0.303 & 0.070 & \textbf{0.029} & \textbf{0.097} & \textbf{0.196} & \textbf{0.362} & 0.311 & 0.172 & \textbf{0.114} & \textbf{0.191} \\ \hline
    \end{tabular}
    }
    \caption{\textbf{Quantitative Evaluation of IP character edit filtration.} The best results are highlighted in bold, while the second-best is underlined. "Original" represents the original unedited image. An upward arrow indicates that a higher value is preferable for the metric, while a downward arrow suggests that a lower value is preferable. It can be observed that our method shows a significant improvement compared to other methods.}
    \label{tab:ip_quantitative_editing}
\end{table*}

==> table/generation_erasure_IP.tex <==
\begin{table}[ht]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|cc|cc|cc}
    \hline
        ~ & \multicolumn{2}{c|}{Erase Concept} & \multicolumn{2}{c|}{Relate Concept} & \multicolumn{2}{c}{Overall} \\ 
        ~ & $\text{CLIP}_e\downarrow$ & $\text{LPIPS}_e\uparrow$ & $\text{CLIP}_p\uparrow$ & $\text{LPIPS}_p\downarrow$ & $\text{CLIP}_d\uparrow$ & $\text{LPIPS}_d\uparrow$ \\ \hline
        SD v1.4~\cite{rombach2022high} & 0.301 & 0.000 & 0.301 & 0.000 & 0.000 & 0.000 \\ \hline
        ESD~\cite{gandikota2023erasing} & 0.227 & 0.331 & 0.276 & 0.255 & 0.049 & 0.076 \\ 
        SPM~\cite{lyu2024one} & 0.239 & 0.288 & \underline{0.296} & \textbf{0.107} & 0.056 & 0.181 \\ 
        AdvUnlearn~\cite{zhang2024defensive} & \textbf{0.166} & \textbf{0.468} & 0.209 & 0.403 & 0.043 & 0.065 \\ 
        MACE~\cite{lu2024mace} & 0.250 & 0.317 & \textbf{0.298} & \underline{0.134} & 0.048 & \underline{0.184} \\ 
        RECE~\cite{gong2024reliable} & 0.176 & \underline{0.426} & 0.257 & 0.270 & \underline{0.081} & 0.156 \\ 
        Ours & \underline{0.175} & 0.397 & 0.295 & 0.196 & \textbf{0.120} & \textbf{0.201} \\  \hline
    \end{tabular}    }
    \caption{\textbf{Quantitative Evaluation of IP character generation erasure.} The best results are highlighted in bold.}
    \label{tab:ip_quantitative_generation}
\end{table}
